Divide and Conquer: Leveraging Intermediate Feature Representations for Quantized Training of Neural Networks

The deep layers of modern neural networks extract a rather rich set of features as an input propagates through the network. This paper sets out to harvest these rich intermediate representations for quantization with minimal accuracy loss while significantly reducing the memory footprint and compute intensity of the DNN. This paper utilizes knowledge distillation through teacher-student paradigm (Hinton et al., 2015) in a novel setting that exploits the feature extraction capability of DNNs for higher-accuracy quantization. As such, our algorithm logically divides a pretrained full-precision DNN to multiple sections, each of which exposes intermediate features to train a team of students independently in the quantized domain. This divide and conquer strategy, in fact, makes the training of each student section possible in isolation while all these independently trained sections are later stitched together to form the equivalent fully quantized network. Our algorithm is a sectional approach towards knowledge distillation and is not treating the intermediate representation as a hint for pretraining before one knowledge distillation pass over the entire network (Romero et al., 2015). Experiments on various DNNs (AlexNet, LeNet, MobileNet, ResNet-18, ResNet-20, SVHN and VGG-11) show that, this approach -- called DCQ (Divide and Conquer Quantization) -- on average, improves the performance of a state-of-the-art quantized training technique, DoReFa-Net (Zhou et al., 2016) by 21.6% and 9.3% for binary and ternary quantization, respectively. Additionally, we show that incorporating DCQ to existing quantized training methods leads to improved accuracies as compared to previously reported by multiple state-of-the-art quantized training methods.

==> body/background.tex <==
\section{Background}

%
The concept of knowledge distillation enables model reduction by facilitating concise knowledge transfer from a pretrained network (teacher) to a new network (student) that is supposedly more optimized (i.e. smaller in size and/or faster in execution). 
%
In the context of teacher-student paradigm, it turns out that multiple student variants can exist each of which can trade one or more of design aspects.
%
\SetKwComment{Comment}{$\triangleright$\ }{}

\subsection{Teacher-Student Variants}
\niparagraph{Thin \& Shallow Student.}
%
[Hinnton] employed knowledge distillation approach with the goal of obtaining small and fast-to-execute student model. 
%
The student network is trained on a softened version of the final output of a larger teacher network or ensemble of networks. 

\vspace{0.2cm}
\niparagraph{Thin \& Deep Student.}
[Bengio] extended that concept by exploiting intermediate layer as a guide for improved knowledge transfer. 
%
Stemming from understanding that depth is a fundamental aspect of representation learning, [Bengio et all] extend the idea of knowledge distillation based model reduction to allow the training of a student network that is deeper and thinner than the teacher one. 
%
For training, they use intermediate representations from hidden layers as intermediate-level hints in addition to the last output of the larger teach network to improve the training process and final performance of the student. 
 
 \vspace{0.2cm}
 \niparagraph{Quantized (Low Precision) Student.}
Although both methods tend to generate new student versions of the original network that are smaller in one sense or another and consequently faster-to-execute, they both entail coming up with a new network architecture, which is strenuous enough.
%
Our proposed method exploits the effectiveness of knowledge distillation and employs it, for the first time, in the context of network quantization. Thus, the student variant in this case is a quantized (low precision) version of the original teacher (full precision).
%
Figure \ref{fig:kd_vars} illustrates the differences between the above mentioned student variants through high level sketches of the respective training procedure and loss optimization.
%
In the following subsections, we further elaborate on the training procedure and provide more details about the used loss functions for optimization.

\subsection{Training Procedure}
%
The training procedure applies knowledge distillation in a stage-wise fashion (as shown in fig.1).
%
Given a full precision pretrained model (teacher), the network is divided into stages each of which is a set of layers. The output of each stage is passed through a softmax layer to generate a valid output probability distribution that is representative of the stage's intermediate features. 
%
KL divergence is then applied on the respective output probability distribution of each stage to generate a loss function. Optimization is carried out through a stage-wise back-propagation within conventional gradient-based training.
%
Figure \ref{fig:train_proc} summarizes the training pipeline of the proposed method and contrasts it to FitNets method.


\subsection{Intermediate Loss Functions}



%\subsection{Binary Kernel Visualization}




==> body/outline.tex <==
\section{RELEQ for large networks}

- 
%
\begin{itemize}
	\item Table.1  Results: layers weights quantization bitwidths for AlexNet and Resnet-20
	\item Sub-section: Algorithmic Changes (moving from small networks to large networks) Reward per network / reward 			boosting / normalization techniques (mathematical formulas)
	\item Fig.1  Policy evolution (quantization bitwidths probability profiles)
	\begin{itemize}
    		\item X-axis: number of episodes 
	        \item 	Y-axis: selection probability 
        	        \item (a) Without Algorithmic changes for Resnet-20 (divergence behavior, oscillations)
	        \item	(b) With Algorithmic changes for Resnet-20 (convergence)
   	\end{itemize}
\end{itemize}

%
\section{Computation Cost}
\begin{itemize}
\item Sub-section: modified RELEQ formulation; replacing quantization state to computation state
\item Table.1: Results: layers weights quantization bitwidths for AlexNet and Resnet-20 (comparing results (bitwidths) with quantization state vs with computation state. Basically showing how the suggested bitwidths would change considering per layer computation cost into account)
\end{itemize}

%
\section{Proposed new regularization technique (quantization-friendly)}


\begin{itemize}
	\item Sub-section: High level idea / theory / mathematical formulation [DONE]
	\item Fig.1: High level idea / theory [DONE]
	\item Fig.2: Accelerated fine-tuning Results (with and without proposed regularization) 
		Benchmark: CIFAR10 [DONE]
	\item Fig.3: (histogram) Weights evolution towards quantized levels during fine-tuning. For example: 
	\begin{itemize}
    		\item X-axis: weights numerical values 
	        \item 	Y-axis: number of occurrences 
        	        \item (a) Original weight distribution for a particular layer 
	        \item (b) Weights distribution after epoch1 (midway of finetuning)
	        \item (c) Weights distribution after epoch2 or end of finetuning (weights are clustered around quantized levels)
   	\end{itemize}
\end{itemize}




==> body/outlook.tex <==
\section{Accelerated Finetuning}
%
 %\niparagraph{Loss function of neural networks.}
 \paragraph{Loss function of neural networks.}
 %
 Neural networks' loss functions are known to be highly non-convex and generally very poorly understood. It has been empirically verified that loss surfaces for large neural networks have many local minima that are essentially equivalent in terms of test error \cite{DBLP:journals/corr/ChoromanskaHMAL14}, \cite{DBLP:journals/corr/abs-1712-09913}. 
%
Moreover, converging to one of the many good local minima proves to be more useful as compared to struggling to find the global minimum of the accuracy loss on the training set (which often leads to overfitting). This opens up and encourages a possibility of adding extra custom objectives to optimize for (during the training process), in addition to the original one (accuracy loss). The added custom objective could be with the purpose of increasing generalization performance or imposing some preference on the weights values. 
%
Regularization is one of the major techniques that makes use of such facts as discussed in the following subsection.
 
 %


%\niparagraph{Quantization friendly regularization.}
\paragraph{Quantization friendly regularization.}
%
Neural networks often suffer from redundancy of parameterization and consequently they commonly tend to overfit.
%
Regularization is one of the commonly used techniques to enhance generalization performance of neural networks.
%
Regularization effectively constrains weight parameters by adding a term (regularizer) to the objective function that captures the desired constraint in a soft way. This is achieved by imposing some sort of preference on weights updates during the optimization process. As a result, regularization seamlessly leads to unconditionally constrained optimization problem instead of explicitly constrained which, in most cases is much more difficult to solve.
%
The most commonly used regularization technique is known as \textit{weight decay}, which aims to reduce the network complexity by limiting the growth of the weights. It is realized by adding a term to the objective function that penalizes large weight values \cite{Krogh:1991:SWD:2986916.2987033}:
\[ E(w) = E_o(w) + \frac{1}{2} \lambda \sum\limits_{i} {w_i}^2 \]

where $E_o$ is the original loss measure, and $\lambda$ is a parameter governing how strongly large weights are penalized. $w$ is a vector containing all free parameters of the network.
%

%\begin{figure}[t]
%	\centering
%	\subfloat[t][]{\includegraphics[width=0.35\textwidth]{figs/quant_friendly_a.pdf}
%		\label{fig:quant_a}}
%	\subfloat[t][]{\includegraphics[width=0.29\textwidth]{figs/quant_friendly_b.pdf}
%		\label{fig:quant_b}}
%	\subfloat[t][]{\includegraphics[width=0.25\textwidth]{figs/quant_friendly_c.pdf}
%		\label{fig:quant_c}}
%	\caption{Quantization friendly regularization.}
%	\label{fig:sin2_reg}
%\end{figure}



\begin{figure}[t]
\centering
\begin{subfigure}{0.35\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/quant_friendly_a.pdf}
		\caption{some caption}
		\label{fig:quant_a}
\end{subfigure}

\begin{subfigure}{0.29\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/quant_friendly_b.pdf}
	\caption{some caption}
		\label{fig:quant_b}
\end{subfigure}

\begin{subfigure}{0.25\textwidth}
  \centering\includegraphics[width=\textwidth]{figs/quant_friendly_c.pdf}
  \caption{some caption}
	\label{fig:quant_c}
\end{subfigure}
\caption{Quantization friendly regularization.}
\label{fig:sin2_reg}
\end{figure}


{\setlength{\parindent}{0cm}Here, we propose a new type of regularization that is friendly to quantization. The proposed regularization is realized by adding a periodic function (regularizer) to the original objective function, Figure \ref{fig:quant_a}. The periodic regularizer has a periodic pattern of minima that correspond to the desired quantization levels. Such correspondence is achieved by matching the period to the quantization step based on a particular number of bits for a given layer.}
\[ E(w) = E_o(w) + \frac{1}{2} \lambda_{q} \sum\limits_{i} {\sin^{2}\left({\frac {\pi w_i} {2^{-qbits}}}\right)} \]
where $E_o$ is the original loss measure, and $\lambda_q$ is a parameter governing how strongly weight quantization errors are penalized. $w$ is a vector containing all free parameters of the network.
%

For the sake of simplicity and clarity, Figures \ref{fig:quant_b} and \ref{fig:quant_c} depict a geometrical sketch for a hypothetical loss surface (original objective function to be minimized) and an extra regularization term in 2-D weight space. 
For weight decay regularization, in Figure \ref{fig:quant_b}, the faded circular contours show that as we get closer to the origin, the regularization loss is minimized. Optimum solution is achieved by striking a balance between the original loss term and the regularization loss term.
%
In a similar way, Figure \ref{fig:quant_c} shows a representation of the proposed regularization. A periodic pattern of minima pockets is seen surrounding the original optimum point. The objective of the optimization problem is to find the best solution that is the closest to one of those minima pockets where weight values are nearly matching the desired quantization levels, hence the name quantization-friendly.
%

%\niparagraph{Evaluation.}
\paragraph{Evaluation.}
%
To demonstrate the effectiveness of the proposed regularization, Figure \ref{fig:sin2_eval_1} shows a comparison of the validation accuracy for CIFAR-10 using conventional finetuning approach versus finetuning with the proposed approach. It can be noticed that, under same limited amount of retraining steps, medium number of bits seem to benefit the most. Observed performance improvements could differ across different networks and different durations of retraining.
%
It should be noted that, using the proposed regularization approach, the weight updates occur in full precision as opposed to clipping the weights to the quantized values, yet the weights eventually converge to desired quantization levels.
 

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/val_accuracy.pdf}
    \caption{Comparison of validation accuracy of CIFAR-10 after retraining for 10k steps at different quantization bitwidths for weights (assuming same bitwidth for all layers).}		  
    \label{fig:sin2_eval_1}
    \vspace{0.2cm}
\end{figure}




==> body/theory.tex <==
\section{Theoretical guarantees of DCQ}%: Upper bound on accumulated residual quantization error through splitting sections}
%
One issue that arises as a result of the strategy of splitting into sections and training each section separately is accumulation of error residuals through sections which may impact the overall performance of the proposed technique.
%
Here, we theoretically derive an upper bound on the total accumulated error across the resulting subnetworks after splitting using a chaining argument and utilizing Lipschitz continuity.  
A rigorous analysis bounding the Lipschitz constant of a deep network can be found in \cite{virmaux2018lipschitz} for arbitrary networks and \cite{zou2019lipschitz} for particular convolutional networks.  

%
\subsection{Upper Bounding Network-wide Error}\label{Nstage}
%
Let’s consider a feed-forward full precision network with the following function formulation.
\[ f_{fp}(x) = (\phi^{(m)} \circ \ \phi^{(m-1)} \circ  ... \circ \ \phi^{(1)}) (x) \]
%f(x) = (φl ◦ φl−1 ◦ ... ◦ φl-11)(x) 
%
where $\phi^{(i)}$ is a given layer of the network.  
Also, for a given layer, let the quantized layer be denoted $\phi^{(i)}_q$.  If we quantize every layer, we will refer to the fully quantized network $f_q$.

Assume the application of our quantization scheme leads to an error in the output of size $\|\phi^{(i)}(x) - \phi^{(i)}_{q}(x)\|<\delta$. This comes from the quantization error guarantee of the used technique.  
Further, assume that $\phi^{(i)}$ has Lipschitz constant $L_i$.  Every one layer network is always a Lipschitz function, where $L_i$ is always bounded by the norm of the weights matrix (see Appendix~\ref{singlestage} for a full description).
%
Under this model, we can use a simple triangle inequality to get
$\|\phi^{(i)}_q(x) - \phi^{(i)}_{q}(y)\| < L_i \|x-y\| + 2\delta.$  
%
Using this fact, and chaining it together across multiple layers, we are able to bound the pointwise error between the full precision network and the quantized network.
\begin{theorem}\label{qfperror}
Let $f_{fp}$ be an $m$ layer network, and each layer has Lipschitz constant $L_i$.  Assume that quantizing each layer leads to a maximum pointwise error of $\delta_i$, and results in a quantized $m$ layer network $f_q$. 
%Under the same assumptions as Lemma \ref{lipschitz}, 
Then for a point $x\in X$, $f_q$ satisfies
\begin{align*}
    \|f_q(x) - f_{fp}(x)\| \le 3\Delta_{m,L},
\end{align*}
where $\Delta_{m,L} = \delta_m + \sum_{i=1}^{m-1} \left(\prod_{j=i+1}^m L_j\right) \delta_i$.
\end{theorem}
The proof can be found in the Appendix~\ref{appendix:proof}.


As the Lipschitz constant of the network is the product of its individual layers’ Lipschitz constants, $L$ can grow exponentially if $L_i \geq 1$.
%
This is the common case for normal network training \cite{cisse2017parseval}, and thus the perturbation will be amplified for such a network. 
%
Therefore, to keep the Lipschitz constant of the whole network small, we need to keep the Lipschitz constant of each layer $L_i < 1$.   This is often done using regularization or weight clipping \cite{szegedy2013intriguing,bartlett2017spectrally,cisse2017parseval,gouk2018regularisation} to suppress network’s accumulation of error.
%
We call a network with $L_i < 1, \forall i = 1, ..., \ L$ a non-expansive network.
Experimentally, Lipschitz constant of each layer is found empirically by taking $\max_{x,y} \|\phi_i(x)-\phi_i(y)\| / \|\phi_{i-1}(x)-\phi_{i-1}(y)\|$. 
%



%\subsection{Weight Only vs Weight \& Activation Quantization Implications on Error Bounds}
%\subsection{Optimum DCQ Splitting}

\subsection{Lipschitz Constants in Classification Networks}

The Lipschitz constant is traditionally defined for regression problems where $f$ can take arbitrary values on $\mathbb{R}$, but it also has implications for classification networks.  For a classification network, the input is labeled data $(x_i, y_i)$ for $y_i$ coming from one of $K$ classes.
Then the output $f(x)$ is a function $f:X\rightarrow \mathbb{R}^K$.  Assume $(x_i, y_i)$ satisfies $y_i = k$ and $f$ can perfectly classify $x_i$.  Then if $f$ has a softmax output, the value $f(x_i) = e_k$ for $e_k$ being the unit vector on the $k^{th}$ class.  
A common problem for classification networks is to determine how much one can perturb the data point $x_i$ and maintain the correct classification (i.e., $f(x_i+\eta)_k > 1/2$ for small $\eta$).  For a more general network that isn't softmax, we can define the distance between classifications as $r = \frac{1}{2}\min_{\{i,j : y_i \neq y_j\}} \|y_i - y_j\|_2$.  This reduces to $r=1/2$ for softmax.  And this leads to the following theorem.

\begin{theorem}\label{mainthm}
Let $r= \frac{1}{2}\min_{\{i,j : y_i \neq y_j\}} \|y_i - y_j\|_2$, and let $f_{fp}$ and $f_q$ be the full precision and quantized $m$ layer networks as in Section \ref{Nstage}.  Let $L = \prod_{i=1}^m L_i$ be the Lipschitz constant of $f_{fp}$.  Then for any $(x_i,y_i)$ that $f_{q}$ perfectly classifies and any perturbation $\eta$ such that $\|\eta\| < \frac{r - 2\Delta_{m,L}}{L}$, $f_q$ will also classify $x_i + \eta$ with label $y_i$.

Moreover, if $f_{fp}$ perfectly classifies $x_i$, then for any perturbation $\eta$ such that $\|\eta\| < \frac{r-5\Delta_{m,L}}{L}$, $f_q$ will also classify $x_i + \eta$ with label $y_i$. 
\end{theorem}
The proof can be found in the Appendix~\ref{appendix:proof}.


==> body/theory_old.tex <==
\section{Theoretical guarantees of DCQ: Upper bound on accumulated residual quantization error through splitting sections}
%
One issue that arises as a result of the strategy of splitting into sections and training each section separately is accumulation of error residuals through sections which may impact the overall performance of the proposed technique.
%
Here, we theoretically derive an upper bound on the total accumulated error across the resulting subnetworks after splitting using a chaining argument and utilizing Lipschitz continuity. 
%
\iffalse
\subsection{draft}
We provide a theoretical argument regarding the upper bound on error across sections. For the sake of argument, we consider layer-wise sections.
%
Each layer of the original network has Lipschitz constant $L_i < C\|W_i\|$. where $\|W_i\|$ is the $2-$norm of the weight tensor of layer $i$ and $C$ is a constant proportional to the maximum derivative of the activation function.  This is because 
%
For the first layer, after quantization, the amount any point in the output moves is $\delta$, which comes from the quantization error guarantee of the used technique; thus, we get:
$$ \|f(x)-f(y)\| < L_1 \|x-y\| + 2\delta_1,$$
where f is the output of the first layer after it has been quantized. Now we iterate for each layer with the input from the previous layer, and we get:
\begin{dmath*}
%\|o(x) - o(y)\| < \\ L_m(L_{m-1}( ... (L_1 \|x-y\| + 2\delta_1)...) + 2\delta_{m-1}) + 2\delta_m
\|o(x) - o(y)\| < \\ \left(\prod_{j=1}^m L_j \right) \|x-y\| + 2\delta_m + 2 \sum_{i=1}^{m-1} \left(\prod_{j=i+1}^m L_j\right) \delta_i,
\end{dmath*}
where $o(x)$ is the output of the DNN. A common practice to keep the product of Lipschitz constants small is by keeping the constants small using regularization or weight clipping. So if we quantize a DNN with a small constant, then the error across the entire network is close to just the sum of quantization errors. Experimentally, Lipschitz constant of each layer is found by taking the max of $\|f(x)-f(y)\| / \|x-y\|$. 

The Lipschitz constant above also has implications for classification networks, where the input is labeled data $(x_i, y_i)$ for $y_i$ coming from one of $k$ classes.  Then the output $o(x)$ is a function $o:X\rightarrow \mathbb{R}^k$.  Take $r = \frac{1}{2}\min_{\{i,j : y_i \neq y_j\}} \|y_i - y_j\|_2$.  For standard $k$ label problems without overlap, this leads to $r=1/2$.  Also, take $L = \left(\prod_{j=1}^m L_j \right)$ to be the Lipschitz constant of the unquantized network.  For any point $x$, if it is perturbed by noise $\epsilon$ such that $\|\epsilon\|<r/L$, the resulting point $y=x+\epsilon$ remains in the neighborhood of $x$ and will receive the same classification.  For the quantized network, we must only consider $r_q = r-2\delta_m - 2 \sum_{i=1}^{m-1} \left(\prod_{j=i+1}^m L_j\right) \delta_i$.  Then for any $\epsilon\|<r_q/L$, $x+\epsilon$ will maintain its same classification.
\fi
%
\subsection{Error Upper Bound: Single-stage}
%
We control the neural network’s Lipschitz constant (Szegedy et al., 2013; Bartlett et al., 2017; Cisse et al., 2017) to suppress network’s accumulation of error.
%
Lipschitz constant describes: when input changes, how much does the output change correspondingly. %For a function $\mathcal{F}_1: x \rightarrow y$ , 
For a function $f:X\rightarrow Y$, if it satisfies
% (f(x1), f(x2)) ≤ kDX(x1, x2), ∀x1, x2 ∈ X
\[ \|f(x_1)- f(x_2)\|_Y \leq L\|x_1- x_2\|_X, \ \ \forall \ x_1, x_2 \in X \]
%
for $L\geq 0$, and norms $\|\cdot\|_X$ and $\|\cdot\|_Y$ on their respective spaces, then we call $h$ Lipschitz continuous and  $L$ is the known as the Lipschitz constant of $h$.

Let us consider a sub-network (section) $i$ with full precision weights $W_{fp}$ and corresponding quantized inputs $W_q$, and let the full precision network output be $f_{fp}(x) = \sigma(W_{fp}x)$ for some activation function $\sigma$ and the quantized network output be $f_q(x) = \sigma(W_q x)$.
%
For a one layer network, full precision network $f_{fp}$ has Lipschitz constant $L$, which satisfies 
$$ L\le C_\sigma \|W_{fp}\| \textnormal{ for } C_\sigma = \frac{d\sigma}{dx}$.$$

Assume the application of our quantization scheme leads to an error in the output of size $\|f_{fp}(x) - f_{q}(x)\|<\delta$. This comes from the quantization error guarantee of the used technique.  
%
Under this model, we can use a simple triangle inequality to get:
$$ \|f_q(x)-f_q(y)\| < L \|x-y\| + 2\delta.$$
%




The quantization residual error per section can be controlled if we have a small Lipschitz constant $L$ (in optimal situation we can have $L \leq 1$). 
%
And thus, and the error across the rest of subnetworks will not be amplified, but reduced. Using a chaining argument, we can derive a formulation for the accumulated error residuals across the entire divided network.
%
\subsection{Error Upper Bound: N-stages (Network-wide)}
%
Let’s consider a feed-forward network with the following function formulation.
\[ f(x) = (\phi_l \circ \ \phi_{l-1} \circ  ... \circ \ \phi_1) (x) \]
%f(x) = (φl ◦ φl−1 ◦ ... ◦ φl-11)(x) 
%
where $\phi_i$ can be a linear layer, convolutional layer, pooling, activation functions, etc. Denote the Lipschitz constant of a function $f$ as $Lip(f)$, then for the above network we have
\[ Lip(f) \leq \prod^L_{i=1}Lip(\phi_i) \]
%Lip(f) ≤ product(I=1:m) Lip(φi)
%
As the Lipschitz constant of the network is the product of its individual layers’ Lipschitz constants, $Lip(f)$ can grow exponentially if $Lip(\phi_i) \geq 1$.
%
This is the common case for normal network training (Cisse et al., 2017), and thus the perturbation will be amplified for such a network. 
%
Therefore, to keep the Lipschitz constant of the whole network small, we need to keep the Lipschitz constant of each layer $Lip(\phi_i) < 1$. 
%
We call a network with $Lip(\phi_i) < 1, \forall i = 1, ..., \ L$ a non-expansive network.
%
Using a chaining argument, the overall formulation for the total accumulated error across the entire network (through all sections) can be represented as follows:
\[ h^{l_n}(x) - h^{l_n}(y) \leq \epsilon + L\epsilon + ... +  L^n\epsilon \]
%|h^(l_n ) (x)-h^(l_n ) (y)|<ϵ+Lϵ+…+L^n ~ ϵ
%
\niparagraph{Keeping the Lipschitz constant small.}
\subsection{Weight Only vs Weight \& Activation Quantization Implications on Error Bounds}
\subsection{Optimum DCQ Splitting}



